Horizon-GS: Unified 3D Gaussian Splatting for Large-Scale Aerial-to-Ground Scenes

Seamless integration of both aerial and street view images remains a significant challenge in neural scene reconstruction and rendering. Existing methods predominantly focus on single domain, limiting their applications in immersive environments, which demand extensive free view exploration with large view changes both horizontally and vertically. We introduce Horizon-GS, a novel approach built upon Gaussian Splatting techniques, tackles the unified reconstruction and rendering for aerial and street views. Our method addresses the key challenges of combining these perspectives with a new training strategy, overcoming viewpoint discrepancies to generate high-fidelity scenes. We also curate a high-quality aerial-to-ground views dataset encompassing both synthetic and real-world scene to advance further research. Experiments across diverse urban scene datasets confirm the effectiveness of our method.

==> sec/preliminary.tex <==
\section{Preliminaries} 
% \label{sec:preliminaries}

% \LX{
% In this section, we briefly introduce 3D Gaussian Splatting (3D-GS)\cite{kerbl20233d} and its variants including Scaffold-GS\cite{lu2023scaffold} and 2D Gaussian Splatting (2D-GS)~\cite{huang20242d}, which are considered as base representations in our approach and key benchmarks for comparison for later experiments.
% Each has demonstrated significant advancement and suitability for large-scale scene rendering or reconstruction.
% }



% \section{Preliminaries}
% \label{sec:preliminaries}

% \paragraph{3D Gaussian Splatting}
% \uml{3D Gaussian Splatting~\cite{kerbl20233d} uses anisotropic 3D Gaussian primitives to explicitly represent scenes. This approach achieves comparable rendering quality but with significantly faster rendering speed, as it retains the differentiable properties of volumetric representations while enabling efficient rendering via a tile-based rasterizer. Specifically, each Gaussian primitive $G$ is parametrized by a center $\mu \in \mathbb{R}^3$, a rotation quaternion $q \in \mathbb{R}^4$, a scaling vector $s \in \mathbb{R}^3$, an opacity $\sigma \in [0,1]$ and a color feature $F \in \mathbb{R}^{3×(2l+1)}$. The color feature $F$ is represented using spherical harmonics (SH) with $l$ degrees to model view-dependent color $c \in \mathbb{R}^3$. To render 2D images from the 3D Gaussians, they are first projected to the image plane as 2D Gaussians $G^{\prime}(x)$ and sorted in front-to-back depth order~\cite{zwicker2001ewa}. An $\alpha$-blending technique is then employed to determine the color for each pixel $p$:
% \begin{equation}
%     C\left(p\right)=\sum_{i \in N} c_i \sigma_i \prod_{j=1}^{i-1}\left(1-\sigma_j\right), \quad \sigma_i=\alpha_i G_i^{\prime}(p),
% \end{equation}
% where $N$ represents the ordered primitives that overlap that pixel.}

% \paragraph{Scaffold-GS}
% \uml{To reduce redundancy, Scaffold-GS~\cite{lu2023scaffold} introduces anchors to locally manage the neural Gaussians. From each anchor, $k$ neural Gaussians are emitted. Specifically, the centers of the $k$ neural Gaussians are determined by adding $k$ learnable offsets to the corresponding anchor position. To render the images from the neural Gaussians via the tile-based rasterizer proposed in~\cite{kerbl20233d}, the other properties are decoded by MLPs from the anchor-wise feature and the relative observing positions. This structured representation improves robustness and storage
% efficiency compared to the vanilla 3D-GS.}

% \paragraph{2D Gaussian Splatting}
% \uml{To accurately represent surfaces, 2DGS~\cite{huang20242d} collapses
% the 3D Gaussians into a set of 2D oriented planar Gaussian disks. An adaptive rasterizer is proposed to efficiently render these 2D Gaussians. Additionally, the depth distortion and normal consistency losses are introduced to further enhance the quality of the reconstructions. Finally, a mesh is extracted from a truncated signed distance fusion (TSDF), which fuses the predicted multi-view depth maps from the optimized 2DGS field. }



